Generate Your Counterfactuals: Towards Controlled Counterfactual Generation for Text

Machine Learning has seen tremendous growth recently, which has led to larger adoption of ML systems for educational assessments, credit risk, healthcare, employment, criminal justice, to name a few. The trustworthiness of ML and NLP systems is a crucial aspect and requires a guarantee that the decisions they make are fair and robust. Aligned with this, we propose a framework GYC, to generate a set of counterfactual text samples, which are crucial for testing these ML systems. Our main contributions include a) We introduce GYC, a framework to generate counterfactual samples such that the generation is plausible, diverse, goal-oriented, and effective, b) We generate counterfactual samples, that can direct the generation towards a corresponding condition such as named-entity tag, semantic role label, or sentiment. Our experimental results on various domains show that GYC generates counterfactual text samples exhibiting the above four properties. GYC generates counterfactuals that can act as test cases to evaluate a model and any text debiasing algorithm.

==> 1_ethics.tex <==
\section{Ethics Statement}
We believe that Language Models have been seen to be generating discriminated or biased text. The proposed framework does not support or amplify any such biases and can not be exploited to generate unethical or biased text in any case. Infact, this work helps in generating data to remove bias from text based algorithms. Therefore the work helps in aiding the checks on unethical data or generation and poses no threat of any kind of discrimination.

